Federated singular value decomposition for high dimensional data

Federated learning (FL) is emerging as a privacy-aware alternative to classical cloud-based machine learning. In FL, the sensitive data remains in data silos and only aggregated parameters are exchanged. Hospitals and research institutions which are not willing to share their data can join a federated study without breaching confidentiality. In addition to the extreme sensitivity of biomedical data, the high dimensionality poses a challenge in the context of federated genome-wide association studies (GWAS). In this article, we present a federated singular value decomposition (SVD) algorithm, suitable for the privacy-related and computational requirements of GWAS. Notably, the algorithm has a transmission cost independent of the number of samples and is only weakly dependent on the number of features, because the singular vectors associated with the samples are never exchanged and the vectors associated with the features only for a fixed number of iterations. Although motivated by GWAS, the algorithm is generically applicable for both horizontally and vertically partitioned data.

==> app.tex <==
%!TEX root = vertical.tex

\section{Web Service}\label{sec:app}
Researchers from the biomedical sciences performing GWAS typically rely on ready-made software such as PLINK \cite{Chang2015}. Consequently, a user-friendly tool is required in order to make federated PCA available to these researchers in order to facilitate adoption in practice.

To render the federated PCA algorithm presented in \Cref{sec:algo} accessible to the biomedical community, we have developed a web-based user interface available at \url{https://anonymous.4open.science/r/hyfed-pca-22F6}. The implementation is based on HyFed \cite{nasirigerdeh2021hyfed}, a Python package for privacy-preserving federated web services. To the best of our knowledge, our web tool is the first ready-to-use privacy-preserving implementation of a federated PCA algorithm. It consists of four components: 
\begin{itemize}
\item A client software which runs at the local sites and computes all parameters using local data.
\item An aggregation software which runs on a central server and aggregated the local (noisy) parameters.
\item A compensator module which aggregates the noise such that the true local parameters are hidden from the aggregation software.
\item A web interface which can be used to set up the study. This includes the generation of tokens for all participants to ensure that only authenticated users participate in the study.
\end{itemize}

To protect the local data from reconstruction attacks at the aggregation server, the HyFed backend provides an SMPC-like parameter obfuscation scheme, where noise is added to the intermediate parameters and subtracted from the global parameters. HyFed assumes an honest-but-curious risk model, \ie, assumes that all participants (aggregator, compensator, as well as all clients) strictly adhere to the protocol but try to extract as much information as possible from legally acquired data. For more details, we refer to the original publication \cite{nasirigerdeh2021hyfed}.




==> evil_layout_algorithms.tex <==
%\documentclass{sn-jnl}
%
%\include{preamble}
%\begin{document}
%
%\algnewcommand{\LeftComment}[1]{\Statex \(\triangleright\) \textit {#1}}
%\algnewcommand\algorithmicret{\textbf{Return:}}
%\algnewcommand\Ret{\item[\algorithmicret]}
%
%\begin{algorithm}[ht]
% \caption{Vertical subspace iteration by \cite{Halko_2010}.} \label{alg:subspace-centralised} 
%  \begin{algorithmic}[1]
% \Require{Data matrix $\A\in\mathbb{R}^{m \times n}$, number of eigenvectors $k$.}
% \Ret{Eigenvector matrix $\G \in \mathbb{R}^{n \times k}$ of $\A^\top\A$.}
%% \tcp{Initialize candidate eigenvector matrix of $\A^\top\A$.}
% \State generate $\G_0 \in \mathbb{R}^{n \times k}$ randomly\label{cent:init-start}
% \State $\G_0\gets  \orthonormalize(\G_0)$\label{cent:init-end}
% %\tcp{Initialize iteration counter.}
% \State $i\gets 1$
% \While{termination criterion not met}
% \LeftComment{Update candidate eigenvector matrix of $\A\A^\top$.}
% \State $\H_i = \A\G_{i-1}$\label{cent:while-start}
% \State $\H_i = \orthonormalize(\H_i)$
% %\tcp{Update candidate eigenvector matrix of $\A^\top\A$.}
% \State $\G_i = \A^\top\H_i$ \label{cent:G-update}
% \State $\G_i \gets  \orthonormalize(\G_i)$\label{cent:while-end}
% %\tcp{Increment iteration counter.}
% \State $i\gets i+1$
% \EndWhile
% %\tcp{Return converged eigenvector matrix of $\A^\top\A$.}
% \State $\G \gets \G_i$ 
% \State \Return $\G$ \label{cent:ret}
%
%\end{algorithmic}
% \end{algorithm}
%
%\begin{algorithm}[ht]
%	
%	\caption{Federated Vertical Subspace Iteration. {\color{blue}(Partial) client-side computations are marked in gray.}}
%	\label{alg:subspace-federated}
%	\begin{algorithmic}[1]
%		\Require Partial data matrices $\A^s\in \mathbb{R}^{m \times n^s}$ at sites $s\in[S]$, number of eigenvectors $k$.
%		\Ret Partial eigenvector matrices $\G^s \in \mathbb{R}^{n^s \times k}$ of $\A^\top\A$ at sites $s\in[S]$.
%		
%		\LeftComment{Initialize partial candidate eigenvector matrices of $\A^\top\A$.}
%		\LeftComment{Use approximate subroutine described in \ref{alg:approx-smpc}} 
%		
%		\If{use approximate initialisation}
%		\State $\H_0 \gets \initApprox()$
%		\For{$s\in[S]$}
%		\State $G_0 \gets \A^{s\top} \H_0$ \label{fed-agg:init-start-approx}
%		\EndFor
%		\LeftComment{Use random initialisation if no initial eigenvector is available}
%		\Else
%		
%		\For{$s\in[S]$}
%		\State generate $\G_0^s \in \mathbb{R}^{n^s \times k}$ \label{fed-sub:init-start} randomly\label{fed-agg:init-start}
%		\EndFor
%		\If{use orthonormalization}
%		\LeftComment {Use approach described in \ref{alg:qr-federated}.}
%		\State $\fedOrthonormalize()$\label{fed-sub:orthonormalize}\label{fed-sub:init-end}
%		\EndIf
%		\EndIf
%		
%		
%		
%		
%		\State $i\gets 1$\; %\Comment{Initialize iteration counter.}
%		\While {termination criterion not met}
%		
%		\LeftComment{Update partial candidate eigenvector matrices of $\A\A^\top$.}
%		\For{$s\in[S]$}
%		\State $\H^s_{i} \gets \A^s\G^s_{i-1}$\label{fed-sub:H-start}
%		\EndFor
%		
%		\State $\H_i \gets \sum_{s=1}^S\H_{i}^s$ \label{fed-sub:aggregate-H}
%		\State$\H_i \gets \orthonormalize(\H_i)$\label{fed-sub:H-ortho}\label{fed-sub:H-end}
%		
%		
%		\LeftComment{Update partial candidate eigenvector matrices of $\A^\top\A$.}
%		\For{$s\in[S]$}
%		\State $\G_i^s \gets {\A^s}^\top \H_i$\label{fed-sub:update-G}
%		\EndFor
%		
%		\If{use orthonormalization}
%		\LeftComment{Use approach described in \ref{alg:qr-federated}.}
%		\State $\fedOrthonormalize()$\label{fed-sub:fed-ortho}
%		\EndIf
%		
%		\LeftComment{Increment iteration counter.}
%		\State $i\gets i+1$
%		\EndWhile
%		
%		\For{$s\in[S]$}
%		\State$\G^s\gets \G_i^s$
%		\Return $\G^s$
%		\EndFor
%	\end{algorithmic}
%\end{algorithm}
%
%
%
%\begin{algorithm}[htb]
%	
%	\caption{Federated Gram-Schmidt. {\color{blue}Client-side computations are marked in gray.}}
%	\label{alg:qr-federated}
%	\begin{algorithmic}[1]
%		\Require Data matrices $\V_s$ at sites $s\in[S]$.
%		\Ret Orthonormalized data matrices $\U_s$ at sites $s\in[S]$.
%		
%		\LeftComment{Compute squared norm of first orthogonal vector.}
%		\For{$s\in[S]$\label{gs-fed:init-start}}
%		\State $\u^s_1 \gets \v^s_1$; $n_1^s \gets {\u_1^s}^\top{\u_1^s}$
%		\EndFor
%		
%		
%		\State $n_1 \gets \sum_{s=1}^S n_1^s$ \; \label{gs-fed:init-end}
%		
%		\LeftComment{Orthogonalize all subsequent vectors.}
%		\For{$i \in [k]\setminus\{1\}$}
%		\LeftComment{Compute client residuals for vector being orthogonalized.}
%		\For{$s\in[S]$\label{gs-fed:res-start}}
%		\For{$j \in[i-1]$}
%		\State $r_{ij}^s \gets {\u_j^s}^\top \v_i^s / n_j $
%		\label{fed-gs:res-end}
%		\EndFor
%		\EndFor
%		\LeftComment{Compute global residuals for vector being orthogonalized.}
%		\For{$j\in[i-1]$\label{gs-fed:aggregated-res-start}}
%		\State $r_{ij} \gets \sum_{s=1}^Sr_{ij}^s$\; \label{gs-fed:aggregated-res-end}
%		\EndFor
%		
%		\LeftComment{Orthogonalize the vector and compute squared norm.}
%		\For{$s\in[S]$\label{gs-fed:norm-start}}
%		\State $\u_{i}^s \gets \v_{i}^s - \sum_{j =1}^{i-1} r_{ij} \cdot \u_{j}^s$\label{gs-client:orth}
%		\State $n_i^s \gets {\u_i^s}^\top \u_i^s$\label{gs-fed:norm-end}
%		\EndFor
%		
%		
%		\LeftComment{Compute squared norm of orthogonalized vector.}
%		\State $n_i \gets \sum_{s=1}^S n_i^s$ \; \label{gs-fed:aggregate-norm}
%		\EndFor
%		
%		\LeftComment{After orthogonalization, scale all $k$ vectors to unit norm.}
%		\For{$s\in[S]$\label{gs-fed:scale-start}}
%		\For{$i \in [k]$}
%		\State $\u_i^s \gets \frac{1}{\sqrt{n_i}}\cdot\u_i^s$
%		\EndFor
%		\State $\U^s\gets[\u_1^s\dots \u^k_s]$; 
%		\State \Return $\U^s$\;\label{gs-fed:scale-end}
%		\EndFor
%	\end{algorithmic}
%\end{algorithm}
%
%\end{document}
